Integrated Task Assignment and Path Planning for Capacitated Multi-Agent Pickup and Delivery

Multi-agent Pickup and Delivery (MAPD) is a challenging industrial problem where a team of robots is tasked with transporting a set of tasks, each from an initial location and each to a specified target location. Appearing in the context of automated warehouse logistics and automated mail sortation, MAPD requires first deciding which robot is assigned what task (i.e., Task Assignment or TA) followed by a subsequent coordination problem where each robot must be assigned collision-free paths so as to successfully complete its assignment (i.e., Multi-Agent Path Finding or MAPF). Leading methods in this area solve MAPD sequentially: first assigning tasks, then assigning paths. In this work we propose a new coupled method where task assignment choices are informed by actual delivery costs instead of by lower-bound estimates. The main ingredients of our approach are a marginal-cost assignment heuristic and a meta-heuristic improvement strategy based on Large Neighbourhood Search. As a further contribution, we also consider a variant of the MAPD problem where each robot can carry multiple tasks instead of just one. Numerical simulations show that our approach yields efficient and timely solutions and we report significant improvement compared with other recent methods from the literature.

==> Makefile <==
FICHIER = main

TEXFILES = $(wildcard *.tex) $(wildcard images/*.tex) $(wildcard algo/*.tex) $(wildcard tikz/*.tex) 
BIBFILE  = $(wildcard *.bib)
FIGFILES = $(wildcard images/*.fig)
EPSFILES = $(patsubst %.fig,%.eps,$(FIGFILES))

TMPFILES  = $(wildcard *.aux) $(wildcard *.bbl) $(wildcard *.ps) $(wildcard *.dvi) $(wildcard *.blg) $(wildcard *.toc) $(wildcard *.lof) $(wildcard *.log) $(wildcard *.lot) 
BACKFILES = $(wildcard *.bak) $(wildcard */*.bak) $(wildcard *~) $(wildcard */*~) $(wildcard *.tar.gz)
TRUCFILES = $(wildcard _*)

DOTFILES = $(wildcard *.dot)
PSDOTFILES = $(patsubst %.dot,%.tps,$(DOTFILES))

all: $(FICHIER).pdf

%.pdf: $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) 
	pdflatex $(FICHIER)

#%.pdf: %.ps
#	ps2pdf $<

#%.tps: %.dot
#	dot -Tps -o $@ $<

%.ps:  %.dvi
	dvips -o $@ $< > /dev/null
#	dvips -Pcmz -Pamz -o $@ $< > /dev/null

%.eps: %.fig
	fig2dev -L eps $< $@

%.dvi: _tpsfiles _epsfiles $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) > /dev/null
	pdflatex $(FICHIER) > /dev/null

_tpsfiles: $(PSDOTFILES)
	touch _tpsfiles

%.tps: %.dot
	dot -Tps -o $@ $<

_epsfiles: $(EPSFILES)
	@echo $(EPSFILES) > _epsfiles

clean:
	-rm -f $(EPSFILES) $(BACKFILES) $(PSDOTFILES)
	-rm -f $(TMPFILES)
	-rm -f $(TRUCFILES)
	-rm -f $(FICHIER).pdf

tar: clean
	perl -e '$$line=`date +"\%y-\%m-\%d"`;chomp($$line);`tar cvf $(FICHIER)-$$line.tar *`;`gzip $(FICHIER)-$$line.tar`;';

tardir: clean
	perl -e '$$pwd = `pwd`; my($$path,$$dir) = $$pwd =~ m/(.*\/)(.*)$$/; $$line=`date +"\%y-\%m-\%d"`;chomp($$line);`cd .. ; tar cvf $$dir-$$line.tar $$dir ; gzip $$dir-$$line.tar ; mv $$dir-$$line.tar.gz $$dir`;';

pwd:
	perl -e '$$pwd = `pwd`; print $$pwd;'

touch:
	@touch $(FICHIER).tex
	@echo You touch my ``$(FICHIER)''.

open:
#	@kile $(FICHIER).tex &
#	@texmaker $(FICHIER).tex &
	@emacs $(FICHIER).tex &





==> Multi-robot task assignment and motion planning (1)/Makefile <==
FICHIER = main

TEXFILES = $(wildcard *.tex) $(wildcard images/*.tex) $(wildcard algo/*.tex) $(wildcard tikz/*.tex) 
BIBFILE  = $(wildcard *.bib)
FIGFILES = $(wildcard images/*.fig)
EPSFILES = $(patsubst %.fig,%.eps,$(FIGFILES))

TMPFILES  = $(wildcard *.aux) $(wildcard *.bbl) $(wildcard *.ps) $(wildcard *.dvi) $(wildcard *.blg) $(wildcard *.toc) $(wildcard *.lof) $(wildcard *.log) $(wildcard *.lot) 
BACKFILES = $(wildcard *.bak) $(wildcard */*.bak) $(wildcard *~) $(wildcard */*~) $(wildcard *.tar.gz)
TRUCFILES = $(wildcard _*)

DOTFILES = $(wildcard *.dot)
PSDOTFILES = $(patsubst %.dot,%.tps,$(DOTFILES))

all: $(FICHIER).pdf

%.pdf: $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) 
	pdflatex $(FICHIER)

#%.pdf: %.ps
#	ps2pdf $<

#%.tps: %.dot
#	dot -Tps -o $@ $<

%.ps:  %.dvi
	dvips -o $@ $< > /dev/null
#	dvips -Pcmz -Pamz -o $@ $< > /dev/null

%.eps: %.fig
	fig2dev -L eps $< $@

%.dvi: _tpsfiles _epsfiles $(TEXFILES)
	pdflatex $(FICHIER)
	if grep -q 'citation' $(FICHIER).aux; then if grep -q 'bibdata' $(FICHIER).aux; then bibtex $(FICHIER); fi else rm -f $(FICHIER).bbl; fi
	pdflatex $(FICHIER) > /dev/null
	pdflatex $(FICHIER) > /dev/null

_tpsfiles: $(PSDOTFILES)
	touch _tpsfiles

%.tps: %.dot
	dot -Tps -o $@ $<

_epsfiles: $(EPSFILES)
	@echo $(EPSFILES) > _epsfiles

clean:
	-rm -f $(EPSFILES) $(BACKFILES) $(PSDOTFILES)
	-rm -f $(TMPFILES)
	-rm -f $(TRUCFILES)
	-rm -f $(FICHIER).pdf

tar: clean
	perl -e '$$line=`date +"\%y-\%m-\%d"`;chomp($$line);`tar cvf $(FICHIER)-$$line.tar *`;`gzip $(FICHIER)-$$line.tar`;';

tardir: clean
	perl -e '$$pwd = `pwd`; my($$path,$$dir) = $$pwd =~ m/(.*\/)(.*)$$/; $$line=`date +"\%y-\%m-\%d"`;chomp($$line);`cd .. ; tar cvf $$dir-$$line.tar $$dir ; gzip $$dir-$$line.tar ; mv $$dir-$$line.tar.gz $$dir`;';

pwd:
	perl -e '$$pwd = `pwd`; print $$pwd;'

touch:
	@touch $(FICHIER).tex
	@echo You touch my ``$(FICHIER)''.

open:
#	@kile $(FICHIER).tex &
#	@texmaker $(FICHIER).tex &
	@emacs $(FICHIER).tex &





==> Multi-robot task assignment and motion planning (1)/conclusion210304.tex <==
\section{Conclusion}

In this paper, we have designed two algorithms MCA and RMCA to solve the Multi-agent Pickup and Delivery problem where each robot
can carry multiple packages simultaneously. MCA and RMCA successfully perform task assignment and path planning simultaneously. 
This is achieved by \updated{using the real collision-free costs to guide the multi-task multi-robot assignment process}. Further, we observe that the newly introduced anytime improvement strategy improves solutions substantially.
\finalUpdated{Future work will extend the anytime improvement strategies to refine the agents' routes, and improve the algorithms' completeness on path planning.}

\ignore{
The future research will focuses on the online experiments and improving the anytime improvement strategy to include the refining of path planning result, not only the refining of task assignment result. By doing this we will able to further improve the solution quality.
}


==> Multi-robot task assignment and motion planning (1)/experiments_icra.tex <==
\section{Experiments}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\columnwidth]{warehouse.png}

\caption{A warehouse map with 21 x 35 tiles, where blue tiles are endpoints for tasks, orange tiles are initial locations of the robots, and black tiles are static obstacles.}
\label{figure:warehouse}
\end{figure}

We perform our experiments on a $21 \times 35$ warehouse map as shown in Fig.  \ref{figure:warehouse}, where black tiles are static obstacles, white tiles are corridors, blue tiles represent potential origins and destinations (endpoints) of the tasks, and orange tiles represent 
starting locations of the robots.

For the experiments, we test the performance of the designed algorithms under different instances. Each instance includes a set of packages/tasks with randomly generated origins and destinations and a fleet of robots/agents, where the origin and destination for each task are different\footnote{Our implementation codes of the designed algorithms are available at:\\ https://github.com/nobodyczcz/MCA-RMCA.git}.

% In this part, we assume that all the tasks are initially released for simplicity, although the designed algorithms can handle the scenario where tasks are released dynamically by following the dynamic task assignment mechanism designed in \cite{bai2020event}. 

\subsection{One-shot Experiment}

\updated{
We first evaluate the designed algorithms in an offline manner to test their scalability. Here, we assume that all the tasks are initially released. This helps us to learn how the number of tasks and other parameters influence the algorithms' performance, and how many tasks our algorithm can process in one assignment time instant.}
\subsubsection{Relative TTD and Runtime}
The first experiment compares variants of methods for different numbers of agents 
and different capacities of agents.
We compare two decoupled versions of the algorithms, where we first complete the task assignment before doing any route planning.  In these variants we use optimal path length as the distance metric while performing task assignment.  We consider two variants: decoupled MCA (MCA-pbs) where we simply assign tasks to the agent which will cause the least delay (assuming optimal path length travel), 
and decoupled RMCA  (RMCA(r)-pbs) where we assign the task with maximum relative regret to its first choice.  
The routing phase uses PBS~\cite{PBS} to rapidly find a set of collision-free routes for the agents given the task assignment.
We compare three coupled approaches:
\ignore{For all of these methods the current travel times are used to compute travel cost. 
}
MCA uses greedy task assignment, while 
RMCA instead uses maximum (absolute or relative) regret to determine which task to assign first.
\ignore{
We consider two forms of regret: absolute regret where which is simply the difference in travel delay
for the first and second options, and relative regret which is defined as the travel delay of the second best option divided by the first option.}
For each number of tasks, each number of agents (Agents) and each capacity (Cap), we randomly generate 25 instances. Each task in each instance randomly selects two endpoints (blue tiles in Fig. \ref{figure:warehouse}) as the start and goal locations for the task.


Fig. \ref{mca_rmca_delay} shows the algorithms' relative TTD. The relative TTD is defined as real TTD minus the TTD of RMCA(r) when ignoring collisions. 
\updated{The reason we use relative TTD as a baseline is that the absolute TTD values in one-shot experiment are very large numbers varying in a relative small range. If using absolute TTD values, it is hard to distinguish the performance difference of algorithms in plots.}
Overall we can see that the decoupled methods are never the best, thus justifying that we want to solve this problem in a coupled manner instead of separate task assignment and routing. For Cap$=1$, MCA is preferable since we cannot modify the route of an agent already assigned to a task to take on a new task and regret is not required.
For Cap$=3$, RMCA(r) eventually becomes the superior approach as the number of agents grows. 
When Cap$=5$, RMCA(r) is clearly the winner. 
Interestingly, the absolute regret based approach RMCA(a) does not perform well at all.
\finalUpdated{This may be because the numbers of tasks assigned to the individual
agents by RMCA(a) are far from even, and the resulting travel delay changes greatly when agents are assigned with more tasks. In other words, RMCA(a) prefers to assign tasks to agents with more tasks.}
\ignore{This may be because the regret comparison, while correct for the current state of agents with their existing tasks, is misleading since the travel delay resulting from RMCA(a) changes greatly when agents with more tasks.} 
The relative regret is more stable to these changes.



\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{mca_rmca_s.png}

\caption{Mean relative TTD versus number of tasks on different numbers of agents and different capacity values.}
\label{mca_rmca_delay}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{runtime_s.png}
\caption{Average runtime versus number of tasks on different numbers of agents and different capacity values. }
\label{fig:runtime}
\end{figure}

\begin{table}
\centering
\caption{Mean Relative TTD of Anytime MCA/RMCA on 500 tasks.}
% \begin{subtable}
% \centering
\setlength{\tabcolsep}{2pt}
\resizebox{0.85\columnwidth}{!}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
	        \multirow{3}{*}{Cap}  & \multirow{3}{*}{Agents} & \multirow{3}{*}{RMCA(r)} & \multicolumn{3}{c|}{ RMCA(r)+DR} &
	        \multicolumn{3}{c|}{ RMCA(r)+DW} & \multicolumn{3}{c|}{ RMCA(r)+DM}
	        \\
	        \cline{4-12}
             &&& \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} \\
			 \cline{4-12}
             &&& 1 & 3 & 5 & 1 & 3 & 5 & 1 & 3 & 5  \\
			\hline
			1 & 20 & 2762 & 1800 & \textbf{1687} & 1752 & 2108 & 2025 & 2088 & 2714 & 2565 & 2454 \\
			 & 30 & 2871 & 2009 & \textbf{1902} & 1915 & 2276 & 2215 & 2363 & 2827 & 2743 & 2652 \\
			 & 40 & 2876 & 2089 & \textbf{2031} & 2060 & 2367 & 2328 & 2471 & 2836 & 2788 & 2701 \\
			 & 50 & 2906 & 2195 & 2173 & \textbf{2199} & 2481 & 2469 & 2604 & 2887 & 2830 & 2791 \\
			\hline
			3 & 20 & 1085 & 529 & 487 & 470 & 530 & \textbf{416} & 464 & 1058 & 980 & 861 \\
			 & 30 & 1132 & 765 & 710 & 689 & 729 & \textbf{654} & 686 & 1116 & 1074 & 1023 \\
			 & 40 & 1155 & 819 & 798 & \textbf{781} & 812 & 791 & 792 & 1148 & 1129 & 1108 \\
			 & 50 & 1193 & 888 & \textbf{856} & 858 & 875 & 862 & 877 & 1187 & 1171 & 1131 \\
			\hline
			5 & 20 & 726 & 370 & 331 & 319 & 311 & \textbf{253} & 260 & 698 & 635 & 585 \\
			 & 30 & 757 & 452 & 441 & \textbf{415} & 451 & 420 & 433 & 747 & 718 & 687 \\
			 & 40 & 848 & 536 & 511 & 525 & 511 & 482 & \textbf{480} & 839 & 810 & 782 \\
			 & 50 & 906 & 617 & 623 & 623 & 614 & \textbf{574} & 584 & 899 & 883 & 861 \\
			\hline
% 		\end{tabular}
% 		}
% \end{subtable} 
% %
% \begin{subtable}
% \centering
% (b)
% \resizebox{0.8\columnwidth}{!}{
% 	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
	        \multirow{3}{*}{Cap}  & \multirow{3}{*}{Agents}& \multirow{3}{*}{MCA} & \multicolumn{3}{c|}{MCA+DR} &
	        \multicolumn{3}{c|}{MCA+DW} & \multicolumn{3}{c|}{MCA+DM}
	        \\
	        \cline{4-12}
             &&& \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} \\
			 \cline{4-12}
             &&& 1 & 3 & 5 & 1 & 3 & 5 & 1 & 3 & 5  \\
			\hline
			1 & 20 & 1497 & 850 & 723 & \textbf{715} & 977 & 952 & 976 & 1451 & 1316 & 1252 \\
			 & 30 & 1514 & 927 & 880 & \textbf{873} & 1115 & 1067 & 1138 & 1486 & 1449 & 1412 \\
			 & 40 & 1994 & 1432 & 1406 & \textbf{1376} & 1618 & 1581 & 1696 & 1976 & 1943 & 1908 \\
			 & 50 & 1983 & 1498 & \textbf{1469} & 1480 & 1675 & 1672 & 1769 & 1973 & 1947 & 1915 \\
			\hline
			3 & 20 & 117 & -360 & -395 & -396 & -378 & \textbf{-434} & -428 & 94 & 58 & -21 \\
			 & 30 & 924 & 549 & 510 & 510 & 535 & \textbf{501} & 516 & 913 & 890 & 858 \\
			 & 40 & 1261 & 898 & 868 & \textbf{854} & 879 & 876 & 885 & 1249 & 1227 & 1199 \\
			 & 50 & 1273 & 938 & 925 & \textbf{914} & 931 & 940 & 947 & 1266 & 1245 & 1222 \\
			\hline
			5 & 20 & 748 & 374 & 357 & 337 & 298 & \textbf{276} & 286 & 734 & 689 & 607 \\
			 & 30 & 1197 & 809 & 793 & 778 & 742 & 724 & \textbf{722} & 1178 & 1128 & 1082 \\
			 & 40 & 1367 & 958 & 937 & 966 & 932 & \textbf{899} & 932 & 1347 & 1311 & 1258 \\
			 & 50 & 1266 & 922 & 896 & 915 & 888 & 889 & \textbf{877} & 1258 & 1230 & 1208 \\
			\hline
		\end{tabular}
		}
% \end{subtable}
	\label{table:anytime_mca}
\end{table}
% \begin{table*}[th]
% \centering
% \caption{TTDs of Anytime Improving Strategies on 500 tasks.(Improving for 60 seconds)}
% \setlength{\tabcolsep}{2.5pt}
% \resizebox{0.8\textwidth}{!}{
% 	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% 			\hline
% 	        \multirow{3}{*}{Capacity}  & \multirow{3}{*}{Number Agents}& \multirow{3}{*}{MCA} & \multirow{3}{*}{RMCA(r)} & \multicolumn{3}{c|}{Destroy Random} &
% 	        \multicolumn{3}{c|}{Destroy Worst} & \multicolumn{3}{c|}{Destroy Multiple} &
% 	        \multirow{2}{*}{TA-Hybrid} &
% 	        \multirow{2}{*}{TA-Hybrid }\\
% 	        \cline{5-13}
%              &&&& \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} & & \\
% 			 \cline{5-13}
%              &&&& 1 & 2 & 5 & 1 & 2 & 5 & 1 & 2 & 5 & 500s & 60s \\
% 			\hline
% 			1 & 20 & 103406 & 105057 & \textbf{81517} & 90093 & 98923 & 101733 & 100903 & 104125 & 104741 & 103225 & 94527 & 128645 & 128667 \\
% 			\hline
% 			1 & 30 & 69207 & 70037 & \textbf{62293} & 65100 & 68356 & 67297 & 68151 & 69494 & 69686 & 69354 & 68163 & 84708 & 85230 \\
% 			\hline
% 			1 & 40 & 51979 & 52814 & \textbf{49685} & 50540 & 52355 & 51253 & 51869 & 52572 & 52800 & 52559 & 51636 & 63491 & 63920 \\
% 			\hline
% 			1 & 50 & 41697 & 42509 & \textbf{41133} & 41442 & 42363 & 41488 & 41701 & 42404 & 42429 & 42391 & 42242 & 50822 & 51191 \\
% 			\hline
% 			3 & 20 & 51257 & 52424 & \textbf{23895} & 29273 & 41167 & 48813 & 48260 & 50437 & 52658 & 51971 & 43382 & -- & -- \\
% 			\hline
% 			3 & 30 & 34330 & 34603 & \textbf{25341} & 27746 & 32622 & 31852 & 32576 & 34145 & 34519 & 34550 & 33044 & -- & -- \\
% 			\hline
% 			3 & 40 & 25485 & 25639 & \textbf{22058} & 23144 & 24915 & 24058 & 24411 & 25142 & 25566 & 25314 & 25255 & -- & -- \\
% 			\hline
% 			3 & 50 & 20485 & 20550 & \textbf{18166} & 19309 & 20371 & 19621 & 19912 & 20332 & 20564 & 20516 & 20503 & -- & -- \\
% 			\hline
% 			5 & 20 & 37675 & 37517 & \textbf{16460} & 20207 & 27787 & 35304 & 34627 & 36049 & 37575 & 36859 & 31834 & -- & -- \\
% 			\hline
% 			5 & 30 & 25368 & 24976 & \textbf{16320} & 19673 & 23157 & 23184 & 23435 & 24345 & 25099 & 24955 & 24048 & -- & -- \\
% 			\hline
% 			5 & 40 & 19085 & 18859 & \textbf{15275} & 16113 & 18188 & 18237 & 18141 & 18618 & 18923 & 18776 & 18677 & -- & -- \\
% 			\hline
% 			5 & 50 & 15684 & 15290 & \textbf{13132} & 14048 & 14962 & 14330 & 14684 & 15026 & 15145 & 15092 & 14897 & -- & -- \\
% 			\hline
% 		\end{tabular}
% 		}
% 	\label{table:anytime}
% \end{table*}

Fig. \ref{fig:runtime} shows the average runtime for the above experiment. The results show that decoupled approaches are advantageous in runtime, especially for instances with a large number of tasks and small capacity. Although RMCA and MCA require more runtime than the decoupled approaches, we demonstrate below that MCA and RMCA are still competitive in runtime compared with other algorithms.

\subsubsection{Anytime Improvement Methods}
\label{sec:anytime-exp}


The second experiment uses any time improvement algorithm to improve the solution from RMCA(r) for $60$ seconds with three neighbourhood destroy strategies:
\finalUpdated{\emph{Destroy random (DR)}, \emph{Destroy worst (DW)} and \emph{Destroy multiple (DM)}}. For each destroy strategy, we run experiments on different destroy group sizes (how many tasks to destroy each time).  The experiment is performed on $25$ instances that each have $500$ tasks with different capacity values and agents' numbers.


\updated{\Cref{table:anytime_mca} shows the results of relative TTD of RMCA(r)/MCA (Relative to the TTD of RMCA(r) that ignores collisions, and the lower the better) under different anytime improvement strategies. The results show that all of the three neighbourhood destroy methods improve the solution quality of RMCA(r) and MCA. We still see that MCA performs better than RMCA(r) when capacity and number of agents are low (The relative TTD of MCA smaller than $0$ means its TTD is smaller than TTD of RMCA(r) that ignores collisions.), even the anytime improvement strategies can not reverse this trend. Overall, destroy random and destroy worst performs better than destroy multiple.
This is not unexpected as simple random neighbourhoods are often very competitive for large neighbourhood search. 
}

% \subsubsection{Comparison with TA-Hybrid}
% \label{sec:makespan}
% The third experiment compares our methods with the approach of TA-Hybrid \cite{liu2019task}.


% \Cref{table:makespan} shows the results of makespan from different settings. Liu~\emph{et al}~\cite{liu2019task}. 
% although clearly this objective is not so informative for the greedy methods.
% Overall we can see that we can provide reasonable solutions in terms of makespan compared with TA-hybrid, but clearly they are better since this is the objective they were designed to tackle. 44
% The inability to handle capacities larger than one means that their solutions are not competitive when capacities are larger, with capacity three or five our solutions, perhaps not unsurprisingly, are much better in terms of makespan.  Hence its clear that, since for the practical case of sortation centres, capacities of agents can be more than one, we do need to have algorithms that take this into account. 
%\ddh{We should evaluate the TA-Hybrid solutions under SoC, since we claim this is right objective}.
  
% \Cref{figure:time_makespan} shows the relative run times of the different approaches. Clearly the approach of  Liu~\emph{et al} has a significant runtime overhead since to perform task assignment they solve a vehicle routing problem using a TSP solver \cite{helsgaun2017extension} with fixed time limit, and they use CBS, which is slow compare to prioritized planning solvers, to perform multi-agent path finding. Of our methods the most efficient is the MCA approach.

% \begin{table*}
% 	\begin{center}
% 	\caption{Makespan of different algorithms.
% 	}
% 	\setlength{\tabcolsep}{2.5pt}
% \resizebox{0.8\textwidth}{!}{
% 		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% 			\hline
% 	        \multirow{3}{*}{Capacity}  & \multirow{3}{*}{Number Agents}& \multirow{3}{*}{MCA} & \multirow{3}{*}{RMCA(r)} & \multicolumn{3}{c|}{Destroy Random} &
% 	        \multicolumn{3}{c|}{Destroy Worst} & \multicolumn{3}{c|}{Destroy Multiple} &
% 	        \multirow{2}{*}{TA-Hybrid} &
% 	        \multirow{2}{*}{TA-Hybrid }\\
% 	        \cline{5-13}
%              &&&& \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} & \multicolumn{3}{c|}{Group Size} & & \\
% 			 \cline{5-13}
%              &&&& 1 & 2 & 5 & 1 & 2 & 5 & 1 & 2 & 5 & 500s & 60s \\
% 			\hline
% 			1 & 20 & 625 & 641 & 759 & 749 & 714 & 641 & 642 & 638 & 637 & 644 & 721 & \textbf{547} & 548 \\
% 			\hline
% 			1 & 30 & 438 & 442 & 514 & 529 & 489 & 447 & 447 & 449 & 447 & 453 & 475 & \textbf{371} & 373 \\
% 			\hline
% 			1 & 40 & 338 & 346 & 388 & 387 & 369 & 352 & 352 & 350 & 350 & 352 & 373 & \textbf{287} & 288 \\
% 			\hline
% 			1 & 50 & 273 & 285 & 303 & 311 & 297 & 292 & 289 & 288 & 289 & 292 & 302 & \textbf{236} & 240 \\
% 			\hline
% 			3 & 20 & \textbf{299} & 304 & 497 & 475 & 430 & 316 & 343 & 327 & 313 & 315 & 360 & -- & -- \\
% 			\hline
% 			3 & 30 & \textbf{218} & \textbf{218} & 356 & 323 & 292 & 242 & 252 & 236 & 224 & 225 & 241 & -- & -- \\
% 			\hline
% 			3 & 40 & 174 & \textbf{173} & 244 & 235 & 214 & 189 & 189 & 182 & 177 & 181 & 188 & -- & -- \\
% 			\hline
% 			3 & 50 & \textbf{149} & \textbf{149} & 204 & 192 & 169 & 155 & 162 & 153 & 152 & 153 & 157 & -- & -- \\
% 			\hline
% 			5 & 20 & 239 & \textbf{238} & 387 & 372 & 338 & 250 & 263 & 256 & 235 & 237 & 268 & -- & -- \\
% 			\hline
% 			5 & 30 & 174 & \textbf{171} & 287 & 272 & 241 & 187 & 194 & 183 & 174 & 175 & 187 & -- & -- \\
% 			\hline
% 			5 & 40 & \textbf{139} & 140 & 222 & 204 & 176 & 152 & 156 & 149 & 148 & 148 & 152 & -- & -- \\
% 			\hline
% 			5 & 50 & 124 & \textbf{122} & 174 & 160 & 147 & 128 & 134 & 127 & 126 & 126 & 133 & -- & -- \\
% 			\hline
% 		\end{tabular}
% 		}
% 	\end{center}
% 	\label{table:makespan}
% \end{table*}




% \begin{figure*}[t]
% \centering
% \includegraphics[width=1\textwidth]{time_makespan.png}

% \caption{Mean running time comparison with TA-Hybrid algorithm. }
% \label{figure:time_makespan}
% \end{figure*}

\updated{
\subsection{Lifelong Experiment}
}
%\color{red}
In this part, we test the performance of RMCA(r) in a lifelong setting compared with the TPTS and CENTRAL algorithms in  \cite{ma2017lifelong}. The MAPD problem solved by TPTS and CENTRAL
assumes that each agent can carry a maximum of one package at a time, and the objective is to minimize the makespan. 
This objective is somewhat misleading when we
consider the continuous nature of the underlying problem
where new tasks arrive as the plan progresses. As a result, minimizing TTD might be a better objective since it may help in optimizing the total throughput of the system by trying to make agents idle as soon as possible, whereas with makespan
minimization all agents can be active until the last time point.



At each timestep, after adding newly released tasks to the unassigned task set $\mathcal P^u$, the system performs RMCA(r) on current assignments set $\mathcal A$, and runs the anytime improvement process on all released tasks that are not yet picked up. The RMCA(r) uses the anytime improvement strategy of destroy random with a group size of $5$. As the anytime improvement triggers at every timestep when new tasks arrive, and involves all released yet unpicked up tasks, we set the improvement time as $1$ second in each run. 



We generate $25$ instances with $500$ tasks. For each instance, we use different task release frequencies ($f$): $0.2$ (release $1$ task every $5$ timestep), $2$ and $10$ ($10$ tasks are released each timestep). For each task release frequency, we test the performance of the algorithms under different agent capacities (Cap) and different numbers of agents (Agents).




%\color{black}

   


\begin{table}
\centering
	\caption{Lifelong Experiment on different algorithms.}
	\setlength{\tabcolsep}{0.5pt}
\resizebox{0.9\columnwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
	        \multirow{2}{*}{$f$} & \multirow{2}{*}{Cap}  & \multirow{2}{*}{Agents}&
	        \multicolumn{3}{c|}{RMCA(r) Anytime} &
	        \multicolumn{3}{c|}{CENTRAL} &
	        \multicolumn{3}{c|}{TPTS} \\
	        \cline{4-12}
	        
	        & & & TTD & Makespan &  T/TS & TTD & Makespan &  T/TS & TTD & Makespan &  T/TS \\
	        
			\hline
			0.2 & 1 & 20 & \textbf{3138} & \textbf{2526} & 0.205 & 4365 & 2528 & 0.364 & 3645 & 2528 & \textbf{0.103} \\
			 &  & 30 & \textbf{2729} & \textbf{2525} & \textbf{0.208} & 3864 & 2527 & 0.762 & 3002 & 2526 & 0.242 \\
			 &  & 40 & \textbf{2297} & \textbf{2523} & \textbf{0.210} & 3572 & 2527 & 1.300 & 2646 & 2525 & 0.442 \\
			 &  & 50 & \textbf{2176} & \textbf{2523} & \textbf{0.214} & 3394 & 2525 & 1.945 & 2456 & 2524 & 0.710 \\
			\cline{2-12}
			 & 3 & 20 & 3056 & 2526 & 0.207 & -- & -- & -- & -- & -- & -- \\
			 & & 30 & 2661 & 2525 & 0.210 & -- & -- & -- & -- & -- & -- \\
			 & & 40 & 2223 & 2523 & 0.216 & -- & -- & -- & -- & -- & -- \\
			& & 50 & 2121 & 2523 & 0.219 & -- & -- & -- & -- & -- & -- \\
			\cline{2-12}
			 & 5 & 20 & 3056 & 2526 & 0.207 & -- & -- & -- & -- & -- & -- \\
			&  & 30 & 2661 & 2525 & 0.211 & -- & -- & -- & -- & -- & -- \\
		     &  & 40 & 2223 & 2523 & 0.217 & -- & -- & -- & -- & -- & -- \\
		     &  & 50 & 2121 & 2523 & 0.219 & -- & -- & -- & -- & -- & -- \\
			\hline
% 			0.5 & 1 & 20 & \textbf{3890} & \textbf{1034} & 0.509 & 5010 & 1036 & 0.115 & 6230 & 1040 & \textbf{0.114} \\
% 			 &  & 30 & \textbf{2862} & \textbf{1030} & 0.514 & 4006 & 1034 & 0.355 & 4653 & 1036 & \textbf{0.348} \\
% 			 &  & 40 & \textbf{2372} & \textbf{1029} & \textbf{0.520} & 3543 & 1034 & 0.720 & 3928 & 1035 & 0.567 \\
% 			 &  & 50 & \textbf{2209} & \textbf{1029} & \textbf{0.531} & 3313 & 1033 & 1.069 & 3663 & 1034 & 0.981 \\
% 			\cline{2-12}
% 			 & 3 & 20 & 3543 & 1032 & 0.514 & -- & -- & -- & -- & -- & -- \\
% 			 &  & 30 & 2712 & 1030 & 0.519 & -- & -- & -- & -- & -- & -- \\
% 			 &  & 40 & 2258 & 1029 & 0.526 & -- & -- & -- & -- & -- & -- \\
% 			 &  & 50 & 2114 & 1029 & 0.535 & -- & -- & -- & -- & -- & -- \\
% 			\cline{2-12}
% 			 & 5 & 20 & 3524 & 1033 & 0.514 & -- & -- & -- & -- & -- & -- \\
% 			 &  & 30 & 2700 & 1029 & 0.521 & -- & -- & -- & -- & -- & -- \\
% 			 &  & 40 & 2258 & 1029 & 0.526 & -- & -- & -- & -- & -- & -- \\
% 			 &  & 50 & 2114 & 1029 & 0.536 & -- & -- & -- & -- & -- & -- \\
% 			\hline
			2 & 1 & 20 & \textbf{65938} & 626 & 0.489 & 75294 & \textbf{610} & 0.125 & 82734 & 639 & \textbf{0.022} \\
			&  & 30 & \textbf{30317} & \textbf{436} & 0.705 & 37327 & 446 & 0.284 & 47252 & 490 & \textbf{0.099} \\
		    &  & 40 & \textbf{13945} & \textbf{344} & 0.884 & 19930 & 376 & 0.426 & 30491 & 413 & \textbf{0.273} \\
			&  & 50 & \textbf{6279} & \textbf{300} & 1.022 & 11185 & 328 & \textbf{0.615} & 21853 & 377 & 0.660 \\
			\cline{2-12}
			 & 3 & 20 & 17904 & 349 & 0.791 & -- & -- & -- & -- & -- & -- \\
			 &  & 30 & 7504 & 302 & 0.933 & -- & -- & -- & -- & -- & -- \\
			&  & 40 & 4644 & 291 & 0.999 & -- & -- & -- & -- & -- & -- \\
			&  & 50 & 3475 & 290 & 1.045 & -- & -- & -- & -- & -- & -- \\
			\cline{2-12}
			 & 5 & 20 & 12711 & 320 & 0.860 & -- & -- & -- & -- & -- & -- \\
			 &  & 30 & 7005 & 299 & 0.942 & -- & -- & -- & -- & -- & -- \\
			 &  & 40 & 4670 & 291 & 1.002 & -- & -- & -- & -- & -- & -- \\
			 &  & 50 & 3463 & 288 & 1.053 & -- & -- & -- & -- & -- & -- \\
			\hline
			10 & 1 & 20 & \textbf{106290} & 624 & 0.142 & 116357 & \textbf{587} & 0.421 & 125374 & 626 & \textbf{0.025} \\
			 &  & 30 & \textbf{68166} & 435 & 0.210 & 76934 & \textbf{419} & 1.062 & 86267 & 462 & \textbf{0.086} \\
			 &  & 40 & \textbf{49140} & 338 & 0.284 & 56896 & \textbf{337} & 2.426 & 66171 & 383 & \textbf{0.238} \\
			 &  & 50 & \textbf{38050} & \textbf{280} & \textbf{0.362} & 45170 & 288 & 2.828 & 55409 & 339 & 0.559 \\
			\cline{2-12}
			 & 3 & 20 & 52771 & 322 & 0.209 & -- & -- & -- & -- & -- & -- \\
			 &  & 30 & 31832 & 226 & 0.305 & -- & -- & -- & -- & -- & -- \\
			 &  & 40 & 21651 & 179 & 0.404 & -- & -- & -- & -- & -- & -- \\
			 &  & 50 & 15851 & 153 & 0.521 & -- & -- & -- & -- & -- & -- \\
			\cline{2-12}
			 & 5 & 20 & 36790 & 247 & 0.271 & -- & -- & -- & -- & -- & -- \\
			 &  & 30 & 21723 & 176 & 0.384 & -- & -- & -- & -- & -- & -- \\
			 &  & 40 & 14970 & 145 & 0.496 & -- & -- & -- & -- & -- & -- \\
			 &  & 50 & 11464 & 129 & 0.613 & -- & -- & -- & -- & -- & -- \\
			\hline
		\end{tabular}
		}
	\label{table:lifelong}

\end{table}
 
\begin{table}
	\begin{center}
	\caption{t-test compares RMCA(r) to CENTRAL and TPTS}
	\label{table:t_test}
    \resizebox{0.8\columnwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|}
			\hline
	          & \multicolumn{2}{c|}{CENTRAL} & \multicolumn{2}{c|}{TPTS} \\
	         \hline
	          & TTD & Makespan & TTD & Makespan \\
			\hline
	         t-score & -17.01 & -0.06 & -22.43 & 1.83 \\
			\hline
	         p-value & $3.47\times 10^{-53}$ & $ 0.95 $ & $ 2.89 \times 10^{-81}$ & $0.06$\\
			\hline
		\end{tabular}
		}
		\end{center}

\end{table}


\subsubsection{Result}
\Cref{table:lifelong} shows that RMCA(r) not only optimizes TTD, its makespans are overall close to CENTRAL, and are much better than TPTS. Comparing TTD, CENTRAL and TPTS perform much worse than RMCA(r). This supports our argument that makespan is not sufficient for optimizing the total throughput of the system. In addition, the \finalUpdated{runtime per timestep (T/TS)} shows that RMCA(r) gets a better solution quality while consuming less runtime on each timestep compared with CENTRAL. A lower runtime per timestep makes RMCA(r) better suited to real-time lifelong operations. Furthermore, by increasing the capacity of robots, both total travel delay and makespan are reduced significantly, which increases the throughput and efficiency of the warehouse.



\subsubsection{T-Test on TTD and Makespan}
We evaluate how significant is the solution quality of RMCA(r) with respect to CENTRAL and TPTS by performing t-test with significance level of $0.1$ on the normalized TTD and normalized makespan for experiments with robots' Cap$=1$. 
The \emph{normalized TTD} is defined as $\frac{TTD \cdot N_a}{N_t \cdot f}$
%$TTD \div N_t \times N_a \div f $, 
where $N_t$ is the number of tasks, $N_a$ is the number of agents and $f$ is the task frequency. This definition is based on the observation that increasing $N_a$ decreases TTD, and increasing $N_t$ and $f$ increases TTD. Similarly \emph{normalized makespan} is $\frac{makespan \cdot N_a \cdot f}{N_t}$
%$makespan \div N_t \times N_a \times f$
(where now increasing $f$ decreases makespan). 
\Cref{table:t_test} shows the $t$-score and $p$-value for the null hypotheses that RMCA(r) and the other methods are identical. The results show that RMCA(r) significantly improves the normalized TTD compared with CENTRAL and TPTS and improves the normalized makespan compared with TPTS.
